Comparative study of space filling curves for cache oblivious TU Decomposition

We examine several matrix layouts based on space-filling curves that allow for a cache-oblivious adaptation of parallel TU decomposition for rectangular matrices over finite fields. The TU algorithm of \cite{Dumas} requires index conversion routines for which the cost to encode and decode the chosen curve is significant. Using a detailed analysis of the number of bit operations required for the encoding and decoding procedures, and filtering the cost of lookup tables that represent the recursive decomposition of the Hilbert curve, we show that the Morton-hybrid order incurs the least cost for index conversion routines that are required throughout the matrix decomposition as compared to the Hilbert, Peano, or Morton orders. The motivation lies in that cache efficient parallel adaptations for which the natural sequential evaluation order demonstrates lower cache miss rate result in overall faster performance on parallel machines with private or shared caches, on GPU's, or even cloud computing platforms. We report on preliminary experiments that demonstrate how the TURBO algorithm in Morton-hybrid layout attains orders of magnitude improvement in performance as the input matrices increase in size. For example, when $N = 2^{13}$, the row major TURBO algorithm concludes within about 38.6 hours, whilst the Morton-hybrid algorithm with truncation size equal to $64$ concludes within 10.6 hours.

==> algs/alg-cluster-head-mobility.tex <==
%\input{algs/alg-keywords}

 \tcp{Cluster Head Mobility}
\BlankLine

\If {cluster-head A cannot hear from any of its cluster-members}{
\If{A hears from CH B and $d^{A}_{B}\leq d_t$}{

A sends \emph{join cluster} to B\\

A becomes a member of cluster B}
}

\ElseIf {A cannot hear any adjacent CH}{ A will maintain its status
as cluster-head}


%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-decode-rowmajor.tex <==
%\input{algs/alg-keywords}

$i$ = $z_{\Theta}$ $\div$ $2^{m}$
\\
$j$ = $z_{\Theta}$ \% $2^{m}$


%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-decoding-mh-dynamic.tex <==
%\input{algs/alg-keywords}

\If {(true)}{Do something} \Else {Do Something else}
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-default-submm.tex <==
%\input{algs/alg-keywords}

\If {(m, n, and p smaller than truncation T)}{ Perform Base Case
Multiplication }
\Else { Calculate sub-matrices start indices\\
        Calculate sub-matrices sizes\\
        Perform eight Recursive Multiplication Calls\\
        }
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-default-submm2.tex <==
%\input{algs/alg-keywords}

\If {(m, n, and p smaller than truncation size T)}{ \For{ i:0 to m }
{
\For{ j:0 to n } { Encode $z_{A}$, index in $S_{A}$, using Sec. \ref{sec:mh_encoding}\\
\For{ k:0 to p } { Encode $z_{B}$, index in $S_{B}$, using Sec. \ref{sec:mh_encoding}\\
Encode $z_{C}$, index in $S_{C}$, using Sec. \ref{sec:mh_encoding}\\
$S_{A}[z_{A}] = S_{A}[z_{A}] + S_{B}[z_{B}] \cdot S_{C}[z_{C}]$} }}}
\Else {
        Perform eight recursive multiplication calls as in Steps \ref{mult_step1} through \ref{mult_step8}\\
        }
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-encode-rowmajor.tex <==
%\input{algs/alg-keywords}

$z_{\Theta}$ = $i$ $\times$ $2^{m}$ + $j$

%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-encoding-mh-dynamic.tex <==
%\input{algs/alg-keywords}

\If {(true)}{Do something} \Else {Do Something else}
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-inplace-submm.tex <==
%\input{algs/alg-keywords}

\If {(m, n, and p smaller than truncation T)}{Perform base case
multiplication} \Else { \For{i: 0...3} { \For{j: 0...3} {\For{k:
0...3} { Calculate current start indices for each
sub-matrix\\
Calculate the number of rows and columns to be included from each
sub-matrix\\
\If{(All dimensions are not zero)}{Perform Recursive Call} } }}}

%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-lower-triangular-inversion.tex <==
%\input{algs/alg-keywords}
$L^{-1} = I$ /*initialize to the identity matrix*/
\\
\For{ i:n to 0 } { \For{ j:i-1 to 0 } { $temp = 0$\\ \For{ k:i to n
} { $temp += L^{-1}[i][k] \cdot L[k][j]$  } $L^{-1}[i][j] = temp \%
2$ } }
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-modified-rectu-general.tex <==
%\input{algs/alg-keywords}

\If {($S_{A^{k}_{t}}$ is \conts in a row-major ordered sub-matrix)}
{/*Perform iterative LU decomposition*/
\\$L \cdot S_{A^{k}_{t}} =  U$
} \Else { Let $A^{k}_{t}$ denote the \alineds sub-matrix resulting
from the recursive division of $A^{k-1}_{t''}$ containing
$S_{A^{k}_{t}}$
\\
Produce the four quadrants $A^{k+1}_{t'} \in \{NW_{A^{k}_{t}},
NE_{A^{k}_{t}}, SW_{A^{k}_{t}}, SE_{A^{k}_{t}}\}$ of $A^{k}_{t}$ as
in Sec. \ref{sec:quads}.
\\
Produce the sub-matrices $\{S'_{A^{k+1}_{t'}}\}$ for each
$A^{k+1}_{t'} \in \{NW_{A^{k}_{t}}, NE_{A^{k}_{t}}, SW_{A^{k}_{t}},
SE_{A^{k}_{t}}\}$ of $A^{k}_{t}$ as in Sec. \ref{sec:quadrants}.
\\
Perform $ModifiedTU(S'_{NW_{A^{k}_{t}}})$ as in Sec. \ref{sec:alg_step1}\\
Update $S'_{NE_{A^{k}_{t}}}$ as in Sec. \ref{sec:alg_step1}\\
Update $S'_{SW_{A^{k}_{t}}}$ as in Sec. \ref{sec:alg_step1}\\
Update $S'_{SE_{A^{k}_{t}}}$ as in Sec. \ref{sec:alg_step1}\\
Perform $ModifiedTU(S'_{SE_{A^{k}_{t}}})$ as in Sec. \ref{sec:alg_step2}\\
Update $S'_{SW_{A^{k}_{t}}}$ as in Sec. \ref{sec:alg_step2}\\
Update $S'_{NE_{A^{k}_{t}}}$ as in Sec. \ref{sec:alg_step2}\\
Update $S'_{NW_{A^{k}_{t}}}$ as in Sec. \ref{sec:alg_step2}\\
Perform $ModifiedTU(S'_{NE_{A^{k}_{t}}})$ as in Sec. \ref{sec:alg_step3}\\
Perform $ModifiedTU(S'_{SW_{A^{k}_{t}}})$ as in Sec. \ref{sec:alg_step3}\\
Update $S'_{NW_{A^{k}_{t}}}$ as in Sec. \ref{sec:alg_step3}\\
Perform $ModifiedTU(S'_{NW_{A^{k}_{t}}})$  as in Sec. \ref{sec:alg_step4}\\
}
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-modified-submm-general.tex <==
%\input{algs/alg-keywords}

\If {($S_{A^{k}_{t}}$, $S_{B^{k}_{u}}$, $S_{C^{k}_{v}}$ are \conts
in row-major ordered sub-matrices)} {/*Perform iterative
multiplication*/
\\$S_{A^{k}_{t}} += S_{B^{k}_{u}} \cdot S_{C^{k}_{v}}$
} \Else { Let $A^{k}_{t}$ denote the \alineds sub-matrix resulting
from the recursive division of $A^{k-1}_{t''}$ containing
$S_{A^{k}_{t}}$; similarly for $B^{k}_{u}$ and $C^{k}_{v}$.
\\
Produce the four quadrants $A^{k+1}_{t'} \in \{NW_{A^{k}_{t}},
NE_{A^{k}_{t}}, SW_{A^{k}_{t}}, SE_{A^{k}_{t}}\}$ of $A^{k}_{t}$ as
in Sec. \ref{sec:quads}.
\\
Do the same for $B^{k}_{u}$ and $C^{k}_{v}$.
\\
\For{(Each $A^{k+1}_{t'} \in \{NW_{A^{k}_{t}}, NE_{A^{k}_{t}},
SW_{A^{k}_{t}}, SE_{A^{k}_{t}}\}$)}{ \For{(Each $B^{k+1}_{u'} \in
\{NW_{B^{k}_{u}}, NE_{B^{k}_{u}}, SW_{B^{k}_{u}},
SE_{B^{k}_{u}}\}$)} {\For{(Each $C^{k+1}_{v'} \in \{NW_{C^{k}_{v}},
NE_{C^{k}_{v}}, SW_{C^{k}_{v}}, SE_{C^{k}_{v}}\}$)} { Produce
$S_{A^{k+1}_{t'}}$, $S_{B^{k+1}_{u'}}$, and $S_{C^{k+1}_{v'}}$
\\
Perform $ModifiedMult(S_{A^{k+1}_{t'}},
S_{B^{k+1}_{u'}},S_{C^{k+1}_{v'}})$ }

} } }
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-modified-submm.tex <==
%\input{algs/alg-keywords}

%\input{algs/alg-keywords}

\If {($S_{A^{k}_{t}}$, $S_{B^{k}_{u}}$, $S_{C^{k}_{v}}$ are \conts
in row-major ordered sub-matrices)} {{/*Perform base case
multiplication*/} \\
\For{ i:0 to m } {\For{ j:0 to n }{Encode $z_{A}$, index in $S_{A^{k}_{t}}$, using Alg. \ref{alg:encode-row-bit}\\\For{ k:0 to p }{Encode $z_{B}$, index in $S_{B^{k}_{u}}$, using Alg. \ref{alg:encode-row-bit}...\\Encode $z_{C}$,  using Alg. \ref{alg:encode-row-bit}\\$S_{A^{k}_{t}}[z_{A}] = S_{A^{k}_{t}}[z_{A}] + S_{B^{k}_{u}}[z_{B}]\cdot S_{C^{k}_{v}}[z_{C}]$...}}}}
\Else{Let $A^{k}_{t}$ denote the
\alineds sub-matrix resulting from the recursive division of
$A^{k-1}_{t''}$ containing $S_{A^{k}_{t}}$; similarly for
$B^{k}_{u}$ and $C^{k}_{v}$.
\\
Find $A^{k+1}_{t'}$ for $t' \in \{0,1,2,3\}$ using \texttt{Produce\_Quads}($A^{k}_{t}$)\\
Find $B^{k+1}_{u'}$ for $u' \in \{0,1,2,3\}$ using \texttt{Produce\_Quads}($B^{k}_{u}$)\\
Find $C^{k+1}_{v'}$ for $v' \in \{0,1,2,3\}$ using \texttt{Produce\_Quads}($C^{k}_{v}$)\\
\For{$t'$: 0...3} {
    Find $S'_{A^{k+1}_{t'}}$ using
    \texttt{Produce\_S'}($A^{k+1}_{t'}$)\\
    \For{$u'$: 0...3} {
        Find $S'_{B^{k+1}_{u'}}$ using
        \texttt{Produce\_S'}($B^{k+1}_{u'}$)\\
        \For{$v'$:0...3} {
            Find $S'_{C^{k+1}_{v'}}$ using \texttt{Produce\_S'}($C^{k+1}_{v'}$)\\

            Find $S_{A^{k+1}_{t'}}$, $S_{B^{k+1}_{u'}}$,
            $S_{C^{k+1}_{v'}}$ using
            \texttt{Produce\_S}($A^{k+1}_{t'},B^{k+1}_{u'},C^{k+1}_{v'}$)\\

            Perform $ModifiedMult(S_{A^{k+1}_{t'}}, S_{B^{k+1}_{u'}}, S_{C^{k+1}_{v'}})$ } }}}

%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-nonrecursive-submm.tex <==
%\input{algs/alg-keywords}

\For{ i:0 to m } { \For{ j:0 to n } { \For{ k:0 to p } { $A[i][j] =
A[i][j] + B[i][k] \cdot C[k][j]$} }}
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-quad-col-offset.tex <==
\If{$Q_{M}$ in west of $M$}{$\varphi_{c_{M}}$ = 0}
\Else{$\varphi_{c_{M}} = c_{N_{M}}$}


==> algs/alg-quad-row-offset.tex <==
\If{$Q_{M}$ in north of $M$}{$\varphi_{r_{M}}$ = 0}
\Else{$\varphi_{r_{M}} = r_{N_{M}}$}


==> algs/alg-rec-inversion.tex <==
%\input{algs/alg-keywords}

\If {(Size smaller than $T$ )} {Perform base case inversion}
\Else {Divide matrix into four quadrants \\
        Perform Recursive Inversion for $NW$ quadrant to find $U^{-1}_{00}$\\
        Perform Recursive Inversion for $SE$ quadrant to find $U^{-1}_{11}$\\
        Perform Recursive Multiplication to find $Temp$\\
        Perform Recursive Multiplication to find $U^{-1}_{01}$
        }

%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-sim-perm.tex <==
%\input{algs/alg-keywords}

\If {(current size is a block)} { map current block to cache\\
\If {(current block  not in cache)} {increment number of misses} }
\Else { \For{each block in row or column major order}{Permutation
Simulation} }

%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-sim-recinv.tex <==
%\input{algs/alg-keywords}

\If {(current size is a block)} { map current block to cache\\
\If {(current block  not in cache)} {increment number of misses} }
\Else {divide size by 2 \\
        Recursive Inversion Simulation for NW quadrant\\
        Recursive Inversion Simulation for SE quadrant\\
        Recursive Multiplication Simulation\\
        Recursive Multiplication Simulation}

%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-sim-reclu.tex <==
%\input{algs/alg-keywords}

\If {(current size is a block)} { map current block to cache\\
\If {(current block  not in cache)} {increment number of misses} }
\Else {divide size by 2 \\
    Recursive LU Simulation for NW\\
    Recursive Multiplication Simulation for NE\\
    Recursive Inversion Simulation for NW\\
    Recursive Multiplication Simulation for N1\\
    Recursive Multiplication Simulation for SW\\
    Recursive Multiplication Simulation for SE\\

    Recursive LU Simulation for SE\\
    Recursive Multiplication Simulation for SW\\
    Recursive Inversion Simulation for SE\\
    Recursive Multiplication Simulation for N2\\
    Recursive Multiplication Simulation for NE\\
    Recursive Multiplication Simulation for NW\\

    Recursive LU Simulation for SW\\
    Recursive LU Simulation for NE\\
    Recursive Inversion Simulation for SW\\
    Recursive Multiplication Simulation for NW\\
    Recursive Multiplication Simulation for N3\\
    Recursive Multiplication Simulation for NW\\

    Recursive LU Simulation for NW\\

    Permutation Simulation by rows\\
    
    Permutation Simulation by columns
}
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/alg-sim-recmm.tex <==
%\input{algs/alg-keywords}

\If {(current size of each matrix involved is a block)} { map each current block to cache\\
\If {(current block  not in cache)} {increment number of misses} }
\Else {divide size by 2 for each matrix \\
    Recursive Multiplication Simulation\\
    Recursive Multiplication Simulation\\
    Recursive Multiplication Simulation\\
    Recursive Multiplication Simulation\\
    Recursive Multiplication Simulation\\
    Recursive Multiplication Simulation\\
    Recursive Multiplication Simulation\\
    Recursive Multiplication Simulation }

%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%


==> algs/modified-submm-general.tex <==
%\input{algs/alg-keywords}

\If {($S_{A^{k}_{t}}$, $S_{B^{k}_{u}}$, $S_{C^{k}_{v}}$ are \conts
in row-major ordered sub-matrices)} {/*Perform iterative
multiplication*/
\\$S_{A^{k}_{t}} += S_{B^{k}_{u}} \cdot S_{C^{k}_{v}}$
} \Else { Let $A^{k}_{t}$ denote the \alineds sub-matrix resulting
from the recursive division of $A^{k-1}_{t^{-1}}$ containing
$S_{A^{k}_{t}}$; similarly for $B^{k}_{u}$ and $C^{k}_{v}$.
\\
Produce the four quadrants $A^{k+1}_{t^{+1}} \in \{NW_{A^{k}_{t}},
NE_{A^{k}_{t}}, SW_{A^{k}_{t}}, SE_{A^{k}_{t}}\}$ of $A^{k}_{t}$ as
in \secref{sec:quads}.
\\
Do the same for $B^{k}_{u}$ and $C^{k}_{v}$.
\\
\For{(Each $A^{k+1}_{t^{+1}} \in \{NW_{A^{k}_{t}}, NE_{A^{k}_{t}},
SW_{A^{k}_{t}}, SE_{A^{k}_{t}}\}$)}{ \For{(Each $B^{k+1}_{u^{+1}}
\in \{NW_{B^{k}_{u}}, NE_{B^{k}_{u}}, SW_{B^{k}_{u}},
SE_{B^{k}_{u}}\}$)} {\For{(Each $C^{k+1}_{v^{+1}} \in
\{NW_{C^{k}_{v}}, NE_{C^{k}_{v}}, SW_{C^{k}_{v}},
SE_{C^{k}_{v}}\}$)} { Identify $S_{A^{k+1}_{t^{+1}}}$,
$S_{B^{k+1}_{u^{+1}}}$, and $S_{C^{k+1}_{v^{+1}}}$
\\
Perform $ModifiedMult(S_{A^{k+1}_{t^{+1}}},
S_{B^{k+1}_{u^{+1}}},S_{C^{k+1}_{v^{+1}}})$ }

} } }
%%%
%%% Local Variables:
%%% mode: latex
%%% End:
%%%

